Dynamic Graph Representation Learning with Neural Networks: A Survey

In recent years, Dynamic Graph (DG) representations have been increasingly used for modeling dynamic systems due to their ability to integrate both topological and temporal information in a compact representation. Dynamic graphs allow to efficiently handle applications such as social network prediction, recommender systems, traffic forecasting or electroencephalography analysis, that can not be adressed using standard numeric representations. As a direct consequence of the emergence of dynamic graph representations, dynamic graph learning has emerged as a new machine learning problem, combining challenges from both sequential/temporal data processing and static graph learning. In this research area, Dynamic Graph Neural Network (DGNN) has became the state of the art approach and plethora of models have been proposed in the very recent years. This paper aims at providing a review of problems and models related to dynamic graph learning. The various dynamic graph supervised learning settings are analysed and discussed. We identify the similarities and differences between existing models with respect to the way time information is modeled. Finally, general guidelines for a DGNN designer when faced with a dynamic graph learning problem are provided.

==> parts/tab_app_datasets_ct.tex <==
\begin{table*}[!ht]\centering
\caption{Commun continuous-time datasets of node or edge-level tasks.}\label{tab: dataset-CT-V} 
\scriptsize
\begin{tabular}{l|l|l|rrrr}\toprule
\toprule
Source & Graph type & Data set & \#Nodes & \#Temporal Edges  & Duration & Publications \\ 
\midrule


%%% A backup version is in backup

% Snap stanford Efeat 172 het
SNAP \cite{snapnets} & Social Network & Reddit\cite{kumar2019predicting} & 11,000 & 672,447  & 30 d & \cite{xu2020inductive} \cite{rossi2020temporal} \cite{kumar2019predicting} \cite{li2020dynamic} \cite{wang2021inductive}\\% Snap stanford

% Snap stanford Efeat 768
 & Social Network & Twitter & 8,861 & 119,872  & 7 d & \cite{rossi2020temporal} \\% Snap stanford

 & Social Network & bitcoin-otc \cite{kumar2016edge} \cite{kumar2018rev2} & 5,881 & 35,592  & (30 d) & \cite{nguyen2018continuous} \cite{qu2020continuous} \cite{pareja2020evolvegcn}\\

 & Social Network & bitcoin-alpha \cite{kumar2016edge} \cite{kumar2018rev2}  & 3,783 & 24,186  & (30 d) & \cite{pareja2020evolvegcn} \cite{pareja2020evolvegcn}\\

 & User-Item Bipartite  & Wikipedia \cite{kumar2019predicting} & 9,227 & 157,474  & 30 d & \cite{xu2020inductive} \cite{rossi2020temporal} \cite{kumar2019predicting} \cite{li2020dynamic} \cite{wang2021inductive}\\

 & User-Item Bipartite & MOOC \cite{kumar2019predicting} & 7,145 & 441,749 & & \cite{wang2021inductive}\\

 & User-Item Bipartite & LastFM \cite{kumar2019predicting} & 2,000 & 1,293,103 & 30 d & \cite{kumar2019predicting} \cite{li2020dynamic}\\
 
 & Internet Interaction & Autonomous systems \cite{leskovec2005graphs} & 6,474 & 13,233  & 30 d &  \\% Snap stanford

 & Citation Network & DBLP \cite{yang2012defining} & 317,080 & 743,70 & & \cite{huang2021temporal} \cite{manessi2020dynamic} \\ 

 & Face-to-face interaction & Resistance \cite{bai2019predicting} \cite{kumar2021deception} & 451 & 3,126,993 & 38 mins& \cite{chen2019lstm} \\%\cite{wang2020generic}
 & (62 graphs) & & & & &  \\%\cite{wang2020generic}
 
 \hline

Network Repository \cite{nr} & Email Network & Radoslaw & 167 & 82.9K & 271.2 d & \cite{nguyen2018continuous} \cite{qu2020continuous} \cite{chen2019lstm}\\%NR 
 
 & Email Network & Enron & 151 & 50,572 &  1137.6 d & \cite{wang2021inductive} \cite{nguyen2018continuous} \cite{qu2020continuous} \cite{chen2019lstm} \cite{hajiramezanali2019variational}
\\% not same ?
 
 & Email Network & email-EU& 986& 332.3K& 803.9 d & \cite{nguyen2018continuous}\\%NR

 & Face-to-face interaction & CONTACT & 274 & 28,200 & 4.0 d& \cite{nguyen2018continuous} \cite{chen2019lstm}\\%NR 
 
 & Face-to-face interaction & HYPERTEXT09 & 113 & 20,800 & 2.5 d& \cite{nguyen2018continuous} \cite{qu2020continuous}\\%NR   


 & Social Network & wiki-Elec & 7.1K & 107K  & 1378.3 d & \cite{nguyen2018continuous} \cite{qu2020continuous}\\ 
\hline

%  & & Industrial & 151 & 50,572 & second &  & \cite{xu2020inductive} \\% NOT AVAILABLE ANYMORE

 
 
 MIT & Physical Proximity & Social Evolution \cite{madan2011sensing} & 83 & 2,016,339  & & \cite{trivedi2019dyrep} \cite{wang2021inductive} \cite{hajiramezanali2019variational} % 791 or 2,016,339 
\\ % realitycommons.media.mit.edu 

KONECT & Social Network & UC Irvine forum \cite{opsahl2009clustering} & 1,899 & 59,835  & & \cite{wang2021inductive}\\ 



%ref:https://openreview.net/pdf?id=HyePrhR5KX p8
%  & Socialnetwork & Github & 12,328 & 166,565 or 604,649 & - & & \cite{trivedi2019dyrep} \\ % Private collected dataset 

% ？ Ryan Rossi and Nesreen Ahmed. 2015. The network data repository with interactive graph analytics and visualization. In Twenty-Ninth AAAI Conference on Artificial Intelligence

Facebook & Social Network & FB-Forum & 899 & 33.7K  & 164.49 d & \cite{nguyen2018continuous} \cite{qu2020continuous} \cite{chen2019lstm}\\ 
%  & & LKML & 2,210 & 422.4K & & 2,436.3 d & \cite{chen2019lstm}\\

%  & face-to-face interaction & comm-f2f-Resistance & 451 & 3,126,993 & \cite{chen2019lstm} \\


Yelp & User-Item Bipartite & YELP & 6,569 & 95,361  & & \cite{huang2021temporal}\\ 



% ? & Bitcointransactions & Elliptic & 203,769 & 234,355 & 49 timesteps & & \cite{pareja2020evolvegcn}\\ 




% feat

%  & Citationnetwork & HEP-TH & 7,980 & 21,036 & Monthly & & \\ 
%  & Communicationnetwork & Autonomous systems & 103-6,474{5} & 13,233 & Daily & & \\ 
%  & Eventsknowledgegraph & GDELT & 14,018 & 31.29M & 15mins & & \\ 
%  & Eventsknowledgegraph & ICEWS & 12498 & 0.67M & Daily & & \\ 
%  & Knowledgegraph & YAGO & 15,403 & 138,056 & Mostlyyearly & & \\ 
%  & Knowledgegraph & Wikidata & 11,134 & 150,079 & Yearly & & \\ 
%  & Socialnetwork & Reddit & 55,863 & 858,49 & Seconds & & \\ 
%  & Socialnetwork & Blog & 5,196 & 171,743 & - & & \\ 
%  & Citationnetwork & Cora^{6} & 2708 & 5429 & - & & \\ 
%  & Socialnetwork & Flicker & 1,715,256 & 22,613,981 & - & & \\ 
%  & Bipartiteratings & MovieLens-10M & 20,537 & 43,760 & Seconds & & \\ 
\bottomrule
\end{tabular}
\end{table*}


%% MANY REFs
%https://arxiv.org/pdf/2101.05974.pdf






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{table*}[!h]\centering
% \caption{DATASETS - Spatial Temporal Graphs}\label{tab: dataset-CT-V} 
% \scriptsize
% \begin{tabular}{l|l|l|rrrrr}\toprule
% \toprule
% Source & Graph type & Data set & \#Nodes & \#Edges & Granuality & Duration & Publications \\ 
% \midrule

% & Traffic Flow & METR-LA & 207 & ?  & ? & 4 months & \cite{li2017diffusion}\\
% & Traffic Flow & PeMS-BAY & 235 & ? & ? & 6 months & \cite{li2017diffusion}\\
% & Traffic Flow & PeMS-BAY & 235 & ? & ? & 7 years & \\


% % niid.go.jp/ & Influenza & Japan-Prefecture & 7 years







% \bottomrule
% \end{tabular}
% \end{table*}

% \break

==> parts/tab_app_notation.tex <==
\begin{table}[ht]\centering%[width=1.0\linewidth,cols=2,pos=ht]
\caption{Commonly used notations.}\label{tbl1}
\scriptsize
\begin{tabular}{lr}\toprule

\toprule
Notations\ \&\ Descriptions\\
\midrule
$|\cdot|$ & The length of a set \\
$G$ & A static graph \\
DG & A dynamic graph \\
$V$ & The set of nodes of a graph \\
$E$ & The set of edges of a graph \\
$T$ & The set of time steps of a graph\\
$\textbf{A}$ & The adjacent matrix a graph \\
% $\textbf{D}$ & The degree matrix a graph \\
$u$ & A certain node $u \in V$ \\
$v$ & A certain node $v \in V$ \\
$i,j$ & The indexes of an event or a node \\
$e$ & A certain edge $e \in E$ \\
$t$ & Time step / timestamp\\
$t^-$ & Latest time step / timestamp < t\\
$\Delta$ & Duration \\
$\delta$ & Modification of an edge \\
$d$ & The dimension of a vector \\

$X$ & The feature of a (dynamic) graph \\
$X_V$ & The node feature of a (dynamic) graph \\
$X_E$ & The edge feature of a (dynamic) graph \\
$Z$ & The encoded hidden states matrix of a\\
    & (dynamic) graph \\

$N_t(v)$ & The set of neighboring nodes of node\\
         & $v$ at time $t$ \\


NN & A neural network \\
$f()$ & NN for encoding DG \\
$f_G()$ & NN for encoding topological information \\
$f_T()$ & NN for encoding temporal information \\

$\theta$ & Learned model parameters \\
$||$ & Vector concatenation \\
$\oplus$ & Element wise sum \\
$\odot$ & Element wise product \\


\bottomrule
\end{tabular}
\end{table}

